A Message Passing Approach for Decision Fusion in Adversarial Multi-Sensor Networks

We consider a simple, yet widely studied, set-up in which a Fusion Center (FC) is asked to make a binary decision about a sequence of system states by relying on the possibly corrupted decisions provided by byzantine nodes, i.e. nodes which deliberately alter the result of the local decision to induce an error at the fusion center. When independent states are considered, the optimum fusion rule over a batch of observations has already been derived, however its complexity prevents its use in conjunction with large observation windows. In this paper, we propose a near-optimal algorithm based on message passing that greatly reduces the computational burden of the optimum fusion rule. In addition, the proposed algorithm retains very good performance also in the case of dependent system states. By first focusing on the case of small observation windows, we use numerical simulations to show that the proposed scheme introduces a negligible increase of the decision error probability compared to the optimum fusion rule. We then analyse the performance of the new scheme when the FC make its decision by relying on long observation windows. We do so by considering both the case of independent and Markovian system states and show that the obtained performance are superior to those obtained with prior suboptimal schemes. As an additional result, we confirm the previous finding that, in some cases, it is preferable for the byzantine nodes to minimise the mutual information between the sequence system states and the reports submitted to the FC, rather than always flipping the local decision.

==> mybibfile <==
@ARTICLE{Vemp13,
author={A. Vempaty and T. Lang and P. Varshney},
journal={IEEE Signal Processing Magazine},
title={Distributed Inference with Byzantine Data: State-of-the-Art Review on Data Falsification Attacks},
year={2013},
month={Sept},
volume={30},
number={5},
pages={65-75}
}


@article{ephraim2002hidden,
  title={Hidden markov processes},
  author={Ephraim, Yariv and Merhav, Neri},
  journal={IEEE Transactions on information theory},
  volume={48},
  number={6},
  pages={1518--1569},
  year={2002},
  publisher={IEEE}
}

@ARTICLE{WSNDDByz,
author={Abdelhakim, M. and Lightfoot, L.E. and Jian Ren and Tongtong Li},
journal={IEEE Transactions on Parallel and Distributed Systems,},
title={Distributed Detection in Mobile Access Wireless Sensor Networks under Byzantine Attacks},
year={2014},
month={April},
volume={25},
number={4},
pages={950-959},
keywords={computer network security;mobile radio;radio access networks;sensor fusion;wireless sensor networks;Byzantine attacks;adaptive data fusion;central limit theorem;distributed detection;entropy-based trust model;false alarm rate;malicious node detection scheme;miss detection constraint;miss detection probability;mobile access wireless sensor networks;near-optimal closed-form solution;reliable data fusion;time-varying attacks;Closed-form solutions;Data integration;Mobile communication;Mobile computing;Reliability;Sensors;Wireless sensor networks;Byzantine attacks;Security in wireless sensor networks;distributed detection},
doi={10.1109/TPDS.2013.74},
ISSN={1045-9219},}

 @ARTICLE(Raw11,
  AUTHOR = "A. S. Rawat and P. Anand and H. Chen and P. K. Varshney",
  TITLE = "Collaborative Spectrum Sensing in the Presence of Byzantine Attacks in Cognitive Radio Networks",
  JOURNAL = "IEEE Transactions on Signal Processing",
  YEAR = "2011",
  VOLUME = "59",
  NUMBER = "2",
  MONTH = "February",
  PAGES = "774-786")


@inproceedings{WSNanomalyDet,
  title={Distributed anomaly detection in wireless sensor networks},
  author={Rajasegarar, Sutharshan and Leckie, Christopher and Palaniswami, Marimuthu and Bezdek, James C},
  booktitle={Proc. of ICCS 2006, 10th IEEE Singapore International Conference on Communication systems},
  pages={1--5},
  year={2006},
  organization={IEEE}
}

@article{WLSH10,
  title={Securing collaborative spectrum sensing against untrustworthy secondary users in cognitive radio networks},
  author={W. Wang and H. Li and Y. Sun and Z. Han},
  journal={EURASIP Journal on Advances in Signal Processing},
  volume={2010},
  pages={4},
  year={2010},
  publisher={Hindawi Publishing Corp.}
}

@ARTICLE{Rawat11,
author={A. S. Rawat and P. Anand and C. Hao and P. K. Varshney.},
journal={IEEE Transactions on Signal Processing},
title={Collaborative Spectrum Sensing in the Presence of Byzantine Attacks in Cognitive Radio Networks},
year={2011},
volume={59},
number={2},
pages={774-786}}

@inproceedings{Zhang2013secure,
  title={Secure crowdsourcing-based cooperative spectrum sensing},
  author={Zhang, Rui and Zhang, Jinxue and Zhang, Yanchao and Zhang, Chi},
  booktitle={Proc. of INFOCOM 2013, IEEE Conference on Computer Communications},
  pages={2526--2534},
  year={2013},
  organization={IEEE}
}

@inproceedings{wang2014secure,
  title={Secure cooperative spectrum sensing and access against intelligent malicious behaviors},
  author={Wang, Wei and Chen, Lin and Shin, Kang G and Duan, Lingjie},
  booktitle={Proc. of INFOCOM 2014, IEEE Conference on Computer Communications},
  pages={1267--1275},
  year={2014},
  organization={IEEE}
}

@article{Mar09,
  title={Distributed detection in the presence of Byzantine attacks},
  author={S. Marano and V. Matta and L. Tong},
  journal={IEEE Transactions on Signal Processing,},
  volume={57},
  number={1},
  pages={16--29},
  year={2009}
  }

@INPROCEEDINGS{DistrDetTree,
author={Kailkhura, B. and Brahma, S. and Varshney, P.K.},
booktitle={IEEE International Conference on Computing, Networking and Communications (ICNC)},
title={Optimal Byzantine attacks on distributed detection in tree-based topologies},
year={2013},
month={Jan},
pages={227-231},
keywords={computational complexity;decision trees;distributed sensors;knapsack problems;radio networks;telecommunication network topology;BKP;bounded knapsack problem;data falsification attacks;decision fusion scheme;distributed detection mechanism;minimum cost Byzantine attacks;node decisions;optimal Byzantine attacks;polynomial time;tree-based topology;Bismuth;Conferences;Decision support systems;Government;Nickel;Silicon;Bounded Knapsack Problem;Byzantine Attacks;Distributed Detection;Tree Topologies},
doi={10.1109/ICCNC.2013.6504085},}

@INPROCEEDINGS{AdvSP,
author={M. Barni and F. P\'erez-Gonz\'alez},
booktitle={2013 IEEE International Conference on Acoustics, Speech and Signal Processing},
title={Coping with the enemy: Advances in adversary-aware signal processing},
year={2013},
pages={8682-8686},
keywords={binary decision diagrams;game theory;signal processing;adversarial machine learning;adversary-aware signal processing;binary decision problem;biometric spoofing;blind sensitivity attack;game-theoretic approach;hill-climbing attack;media forensics;watermarking;Forensics;Games;Sensitivity;Signal processing;Vectors;Watermarking;Game-theory;adversary;binary decision;biometric spoofing;forensics;reputation;watermarking},
doi={10.1109/ICASSP.2013.6639361},
ISSN={1520-6149},
month={May},}

@ARTICLE{TIFSDFByz,
author={A. Abrardo and M. Barni and K. Kallas and B. Tondi},
journal={IEEE Transactions on Information Forensics and Security},
title={A Game-Theoretic Framework for Optimum Decision Fusion in the Presence of Byzantines},
year={2016},
volume={11},
number={6},
pages={1333-1345},
keywords={decision making;game theory;minimisation;numerical analysis;performance evaluation;sensor fusion;telecommunication security;wireless sensor networks;Byzantines;binary decision making;data fusion accuracy improvement;fusion center;game equilibrium point;game theory;malicious nodes;mutual information minimization;numerical simulations;optimum decision fusion;performance evaluation;Cognitive radio;Data integration;Dynamic programming;Error probability;Games;Knowledge engineering;Numerical simulation;Adversarial signal processing;Byzantine nodes;byzantine nodes;data fusion in malicious settings;decision fusion;distributed detection with corrupted reports;dynamic programming;game theory},
doi={10.1109/TIFS.2016.2526963},
ISSN={1556-6013},
month={June},}

@ARTICLE{genlaw,
author={S. M. Aji and R. J. McEliece},
journal={IEEE Transactions on Information Theory},
title={The generalized distributive law},
year={2000},
volume={46},
number={2},
pages={325-343},
keywords={decoding;graph theory;message passing;turbo codes;BCJR algorithm;Baum-Welch algorithm;FFT;GDL;Gallager-Tanner-Wiberg decoding algorithm;Pearl belief propagation algorithm;Shafer-Shenoy probability propagation algorithm;Viterbi algorithm;fast Fourier transform;finite Abelian group;general message passing algorithm;generalized distributive law;junction tree condition;turbo decoding;Artificial intelligence;Decoding;Digital communication;Digital signal processing;Fast Fourier transforms;Information theory;Message passing;Signal processing algorithms;Signal synthesis;Statistical distributions},
doi={10.1109/18.825794},
ISSN={0018-9448},
month={Mar},}

@ARTICLE{genlawnewlook,
author={P. Pakzad and V. Anantharam},
journal={IEEE Transactions on Information Theory},
title={A new look at the generalized distributive law},
year={2004},
volume={50},
number={6},
pages={1132-1155},
keywords={artificial intelligence;iterative decoding;parity check codes;tree codes;turbo codes;GDL;belief propagation;conditional independence;generalized distributive law;graphical model;iterative decoding;junction tree algorithm;lifting;marginal computation;signed measures;triangulation procedure;Artificial intelligence;Extraterrestrial measurements;Graphical models;Iterative algorithms;Iterative decoding;Parity check codes;Random variables;Tree graphs;Turbo codes;Viterbi algorithm;Belief propagation;GDL;conditional independence;generalized distributive law;graphical models;iterative decoding;junction tree;signed measures},
doi={10.1109/TIT.2004.828058},
ISSN={0018-9448},
month={June},}

@ARTICLE{GallagerLDPC,
author={R. Gallager},
journal={IRE Transactions on Information Theory},
title={Low-density parity-check codes},
year={1962},
volume={8},
number={1},
pages={21-28},
keywords={Error-correcting codes;Parity checks;Channel capacity;Communication systems;Data communication;Equations;Error correction codes;Error probability;Information theory;Linear approximation;Maximum likelihood decoding;Parity check codes},
doi={10.1109/TIT.1962.1057683},
ISSN={0096-1000},
month={January},}

@article{verdu1987OptwithMP,
  title={Abstract dynamic programming models under commutativity conditions},
  author={Verdu, Sergio and Poor, H Vincent},
  journal={SIAM Journal on Control and Optimization},
  volume={25},
  number={4},
  pages={990--1006},
  year={1987},
  publisher={SIAM}
}

@article{beliefpropagationAI,
  title={Probabilistic Reasoning in Intelligent Systems, San Mateo, CA},
  author={Pearl, Judea and Kaufmann, M},
  journal={Cal.: Morgan Kaufmann},
  year={1988}
}

@INPROCEEDINGS{Bar13,
author={M. Barni and B. Tondi},
booktitle={Proc. of WIFS'13, IEEE International Workshop on Information Forensics and Security},
title={Multiple-observation hypothesis testing under adversarial conditions},
year={2013},
month={Nov},
address="Guangzhou, China",
pages={91-96}
}

@ARTICLE{Sun12,
author={Yan Sun and Yuhong Liu},
journal={IEEE Signal Processing Magazine},
title={Security of online reputation systems: The evolution of attacks and defenses},
year={2012},
month={March},
volume={29},
number={2},
pages={87-97}
}

@INPROCEEDINGS{CDC14,
author={A. Abrardo and M. Barni and K. Kallas and B. Tondi},
booktitle={53rd IEEE Conference on Decision and Control},
title={Decision fusion with corrupted reports in multi-sensor networks: A game-theoretic approach},
year={2014},
pages={505-510},
keywords={game theory;sensor fusion;adversarial setting;cognitive radio;decision fusion;distributed network monitoring;fusion center;game-theoretic approach;malicious nodes;multi-sensor networks;sensor networks;social networks;Cognitive radio;Data integration;Error probability;Game theory;Games;Reliability;Vectors},
doi={10.1109/CDC.2014.7039431},
ISSN={0191-2216},
month={Dec},}


@ARTICLE{OptFusion,
author={Chair, Z. and Varshney, P.K.},
journal={IEEE Transactions on Aerospace and Electronic Systems},
title={Optimal Data Fusion in Multiple Sensor Detection Systems},
year={1986},
month={Jan},
volume={AES-22},
number={1},
pages={98-101},
keywords={Autocorrelation;Delay effects;Detectors;Frequency;Matched filters;Propagation delay;Radar detection;Sensor fusion;Sensor systems;Surveillance},
doi={10.1109/TAES.1986.310699},
ISSN={0018-9251},}

@book{Rich,
  title={Modern coding theory},
  author={Richardson, Tom and Urbanke, Ruediger},
  year={2008},
  publisher={Cambridge University Press}
}

@book{David,
  title={Information theory, inference and learning algorithms},
  author={MacKay, David JC},
  year={2003},
  publisher={Cambridge university press}
}


@article{Abr1,
  title={Factor graphs and the sum-product algorithm},
  author={Kschischang, Frank R and Frey, Brendan J and Loeliger, H-A},
  journal={IEEE Transactions on Information Theory},
  volume={47},
  number={2},
  pages={498--519},
  year={2001},
  publisher={IEEE}
}



@inproceedings{MaoLDPC,
  title={A heuristic search for good low-density parity-check codes at short block lengths},
  author={Mao, Yongyi and Banihashemi, Amir H},
  booktitle={Communications, 2001. ICC 2001. IEEE International Conference on},
  volume={1},
  pages={41--44},
  year={2001},
  organization={IEEE}
}


@INPROCEEDINGS(KBKV13,
author= "B. Kailkhura and S. Brahma and Y. S. Han and P. K. Varshney",
title= "Optimal Distributed Detection in the Presence of Byzantines",
booktitle="ICASSP 2013, IEEE Int. Conf. on Acoustics, Speech and Signal Processing",
year="2013",
month="27-31 May",
address="Vancouver, Canada")

  @BOOK(Var97,
  AUTHOR="P. K. Varshney",
  TITLE = "Distributed Detection and Data Fusion",
  PUBLISHER = "Springer-Verlag",
  YEAR = "1997")

@ARTICLE{VarshneyHardIso,
author={A. S. Rawat and P. Anand and H. Chen and P. K. Varshney},
journal={IEEE Transactions on Signal Processing},
title={Collaborative Spectrum Sensing in the Presence of Byzantine Attacks in Cognitive Radio Networks},
year={2011},
volume={59},
number={2},
pages={774-786},
keywords={cognitive radio;radio spectrum management;sensor fusion;Byzantine attacks;CR network;cognitive radio networks;collaborative spectrum sensing;data fusion center;data fusion process;optimal attacking strategy;spectrum scarcity;spectrum utilization;transmission opportunity;Cognitive radio;Collaboration;Radiation detectors;Security;Testing;Wireless sensor networks;Byzantine attacks;cognitive radio (CR);network security;spectrum sensing},
doi={10.1109/TSP.2010.2091277},
ISSN={1053-587X},
month={Feb},}


@INPROCEEDINGS{LearnByzantines,
author={Vempaty, A. and Agrawal, K. and Varshney, P. and Hao Chen},
booktitle={Proc. of WCNC'11, IEEE Conf. on Wireless Communications and Networking},
title={Adaptive learning of Byzantines' behavior in cooperative spectrum sensing},
year={2011},
month={March},
pages={1310-1315},
keywords={cognitive radio;communication complexity;cooperative communication;error statistics;probability;spread spectrum communication;Byzantine attacks;Byzantines behavior;adaptive learning;cognitive radio networks;cognitive radio potential malicious behavior;cooperative spectrum sensing;error probability;false alarm probability;fusion rule;Cognitive radio;Convergence;Equations;Joints;Probability;Receiving antennas;Sensors;Byzantine AttacksC;Byzantine Attacksognitive Radio Networks;Spectrum Sensing;ognitive Radio Networks},
doi={10.1109/WCNC.2011.5779320},
ISSN={1525-3511},}


@INPROCEEDINGS{tolerant_scheme,
author={Ruiliang Chen and Jung Min Park and Kaigui Bian},
booktitle={Proc. of INFOCOM 2008, 27th IEEE Conference on Computer Communications},
title={Robust Distributed Spectrum Sensing in Cognitive Radio Networks},
year={2008},
month={April},
pages={-},
keywords={radio networks;sensor fusion;spectral analysers;Byzantine failure;cognitive radio networks;data fusion technique;reputation based mechanism;robust distributed spectrum sensing;sequential probability ratio test;spectrum sensing data falsification attacks;weighted sequential probability ratio test;Chromium;Cognitive radio;Decision support systems;FCC;Interference;Radio spectrum management;Robustness;Sequential analysis;TV;Wireless sensor networks},
doi={10.1109/INFOCOM.2008.251},
ISSN={0743-166X},}



@INPROCEEDINGS{WSNMM1,
author={Tsang-Yi Wang and Chao-Tang Yu},
booktitle={2nd IEEE International Symposium on Wireless Communication Systems},
title={Collaborative Event Region Detection in Wireless Sensor Networks Using Markov Random Fields},
year={2005},
pages={493-497},
keywords={Markov processes;numerical analysis;random processes;sensor fusion;telecommunication network reliability;wireless sensor networks;Markov random fields;channel transmission errors;collaborative event region detection;fusion rule;numerical simulations;sensor faults;sensor fusion technique;sensor nodes;sensor reliability;wireless sensor networks;Algorithm design and analysis;Collaboration;Event detection;Markov random fields;Monitoring;Numerical simulation;Sensor fusion;Sensor phenomena and characterization;Spatial resolution;Wireless sensor networks},
doi={10.1109/ISWCS.2005.1547750},
ISSN={2154-0217},
month={Sept},}

@ARTICLE{WSNMM2,
author={Y. W. P. Hong and A. Scaglione},
journal={IEEE Transactions on Information Theory},
title={Group Testing for Binary Markov Sources: Data-Driven Group Queries for Cooperative Sensor Networks},
year={2008},
volume={54},
number={8},
pages={3538-3551},
keywords={Markov processes;channel allocation;entropy;group theory;queueing theory;recursive estimation;trees (mathematics);wireless sensor networks;binary Markov sources;channel dimension allocation;cooperative sensor networks;data-driven group queries;data-gathering algorithms;group testing;joint entropy;queries sequence;recursive algorithm;scheduling policy;tree-based algorithm;wireless sensor network;Application software;Blood;Entropy;Information retrieval;Performance evaluation;Performance gain;Sensor phenomena and characterization;Source coding;Testing;Wireless sensor networks;Cooperative communications;data gathering in sensor networks;distributed source coding;group testing;multiple access},
doi={10.1109/TIT.2008.926363},
ISSN={0018-9448},
month={Aug},}

@ARTICLE{CRMM1,
author={K. W. Choi and E. Hossain},
journal={IEEE Transactions on Signal Processing},
title={Estimation of Primary User Parameters in Cognitive Radio Systems via Hidden Markov Model},
year={2013},
volume={61},
number={3},
pages={782-795},
keywords={channel estimation;cognitive radio;expectation-maximisation algorithm;hidden Markov models;CR system modeling;EM algorithm;PU signal strength;channel parameter estimation;cognitive radio;equivalence theory;expectation maximization algorithm;hidden Markov model;identifiability analysis;primary user;secondary user;Algorithm design and analysis;Channel estimation;Hidden Markov models;Markov processes;Noise;Parameter estimation;Sensors;Aggregate Markov process;Baum-Welch method;cognitive radio;equivalence;expectation-maximization (EM) algorithm;hidden Markov model;identifiability;parameter estimation},
doi={10.1109/TSP.2012.2229998},
ISSN={1053-587X},
month={Feb},}

@INPROCEEDINGS{CRMM2,
author={I. A. Akbar and W. H. Tranter},
booktitle={IEEE Proceedings of SoutheastCon},
title={Dynamic spectrum allocation in cognitive radio using hidden Markov models: Poisson distributed case},
year={2007},
pages={196-201},
keywords={Poisson distribution;channel allocation;cognitive radio;hidden Markov models;wireless channels;Markov-based channel prediction algorithm;Poisson distributed case;channel behavior;channel state occupancy;cognitive radio networks;dynamic spectrum allocation;hidden Markov models;licensed radio bands;licensed users;radio spectrum management;spectrum holes;spectrum occupancy;spectrum utilization;Chromium;Cognitive radio;Frequency;Heuristic algorithms;Hidden Markov models;Interference;Prediction algorithms;Predictive models;Radio spectrum management;Telecommunication traffic},
doi={10.1109/SECON.2007.342884},
ISSN={1091-0050},
month={March},}

@ARTICLE{CRMM3,
author={T. Jiang and H. Wang and A. V. Vasilakos},
journal={IEEE Journal on Selected Areas in Communications},
title={QoE-Driven Channel Allocation Schemes for Multimedia Transmission of Priority-Based Secondary Users over Cognitive Radio Networks},
year={2012},
volume={30},
number={7},
pages={1215-1224},
keywords={cognitive radio;image coding;multimedia communication;resource allocation;H.264 videos;QoE-driven channel allocation;channel resources;cognitive radio base station;cognitive radio networks;multimedia communication;multimedia secondary users;multimedia transmission;opportunistic spectrum access cognitive radio;primary users;priority service queue;priority-based secondary users;quality of experience;quality-driven wireless multimedia services;spectrum resources;video conferences;Analytical models;Channel allocation;Cognitive radio;Indexes;Markov processes;Multimedia communication;Switches;Cognitive Radio Networks;QoE;channel allocations;multimedia transmission},
doi={10.1109/JSAC.2012.120807},
ISSN={0733-8716},
month={August},}


@ARTICLE{HMMref,
author={L. Rabiner and B. Juang},
journal={IEEE ASSP Magazine},
title={An introduction to hidden Markov models},
year={1986},
volume={3},
number={1},
pages={4-16},
keywords={Fluctuations;Hidden Markov models;Linear systems;Mathematical model;Optimization methods;Pattern matching;Speech processing;Speech recognition;Time varying systems},
doi={10.1109/MASSP.1986.1165342},
ISSN={0740-7467},
month={Jan},}

@INPROCEEDINGS{HMMCR1,
author={K. Kim and I. A. Akbar and K. K. Bae and J. S. Um and C. M. Spooner and J. H. Reed},
booktitle={2nd IEEE International Symposium on New Frontiers in Dynamic Spectrum Access Networks},
title={Cyclostationary Approaches to Signal Detection and Classification in Cognitive Radio},
year={2007},
pages={212-215},
keywords={cognitive radio;feature extraction;frequency-domain analysis;hidden Markov models;pattern matching;radio spectrum management;signal classification;signal detection;HMM;cognitive radio;cycle frequency domain profile;cyclostationary approach;feature extraction;hidden Markov model;pattern matching;signal classification;signal detection;spectrum awareness;threshold-test method;Adaptive signal detection;Chromium;Cognitive radio;Feature extraction;Frequency domain analysis;Hidden Markov models;Pattern classification;Robustness;Signal detection;Signal processing},
doi={10.1109/DYSPAN.2007.35},
month={April},}



@INPROCEEDINGS{VarshDF14,
author={Kailkhura, B. and Brahma, S. and Varshney, P.K.},
booktitle={IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
title={On the performance analysis of data fusion schemes with Byzantines},
year={2014},
pages={7411-7415},
keywords={security of data;sensor fusion;Byzantine attacks;attacker strength;certain fraction;closed form expression;data fusion schemes;fusion center;security performance;Acoustics;Bismuth;Conferences;Decision support systems;Speech;Speech processing;Byzantine Attacks;Data Fusion;Deflection Coefficient;Distributed Detection;Probability of Error},
doi={10.1109/ICASSP.2014.6855040},
month={May},}

